SH2: Self-Highlighted Hesitation Helps You Decode More Truthfully

Large language models (LLMs) demonstrate great performance in text generation. However, LLMs are still suffering from hallucinations. In this work, we propose an inference-time method, Self-Highlighted Hesitation (SH2), to help LLMs decode more truthfully. SH2 is based on a simple fact rooted in information theory that for an LLM, the tokens predicted with lower probabilities are prone to be more informative than others. Our analysis shows that the tokens assigned with lower probabilities by an LLM are more likely to be closely related to factual information, such as nouns, proper nouns, and adjectives. Therefore, we propose to ''highlight'' the factual information by selecting the tokens with the lowest probabilities and concatenating them to the original context, thus forcing the model to repeatedly read and hesitate on these tokens before generation. During decoding, we also adopt contrastive decoding to emphasize the difference in the output probabilities brought by the hesitation. Experimental results demonstrate that our SH2, requiring no additional data or models, can effectively help LLMs elicit factual knowledge and distinguish hallucinated contexts. Significant and consistent improvements are achieved by SH2 for LLaMA-7b, LLaMA2-7b and Mistral-7b on multiple hallucination tasks.

==> figText/parsing-mistral.tex <==
\begin{figure*} [t]
    \centering
    \includegraphics[width=1.01\linewidth]
    {images/parsing-mistral.pdf}
    \caption{The normalized top-$\eta$ recall for different POS tags by LLaMA-7b.}
    \label{fig-parsing-mistral}
\end{figure*}



==> hai.tex <==
sec 3.2

From Figure~\ref{fig-parsing} we observe that \textbf{content words} such as adjectives (JJ), nouns (NN), proper nouns (NNP), adverbs (RB) and conjugated verbs  (VBD, VBG, VBP) are more frequent in the hardest words we extract, as the light color in the heatmap indicates. On the other hand, \textbf{function words} such as conjunctions (CC), determiners (DT) and prepositions (IN) are less frequent, as indicated by the darker colors.\footnote{The base form of the verbs (VB) seems to be an exception. We conjecture that VBs have less information load than conjugated verb forms as the latter also encode tense, aspect and other information about the verb. } 
This suggests our method tends to pick out words that carry more content, rather than those that serve as grammatical functions,
which intuitively could help the model to focus on factual information. 
Our method can thus be understood as a way to ``reiterate'' the content words to LLMs, potentially making them less likely to hallucinate, the effect of which will be evaluated in our experiments. 

